Quantized Compressed Sensing by Rectified Linear Units

This work is concerned with the problem of recovering high-dimensional signals $\mathbf{x} \in \mathbb{R}^n$ which belong to a convex set of low-complexity from a small number of quantized measurements. We propose to estimate the signals via a convex program based on rectified linear units (ReLUs) for two different quantization schemes, namely one-bit and uniform multi-bit quantization. Assuming that the linear measurement process can be modelled by a sensing matrix with i.i.d. subgaussian rows, we obtain for both schemes near-optimal uniform reconstruction guarantees by adding well-designed noise to the linear measurements prior to the quantization step. In the one-bit case, we show that the program is robust against adversarial bit corruptions as well as additive noise on the linear measurements. Further, our analysis quantifies precisely how the rate-distortion relationship of the program changes depending on whether we seek reconstruction accuracies above or below the noise floor. The proofs rely on recent results by Dirksen and Mendelson on non-Gaussian hyperplane tessellations. Finally, we complement our theoretical analysis with numerical experiments which compare our method to other state-of-the-art methodologies.

==> sec_Acknowledgements.tex <==
H.C.J., J.M.\ and L.P. acknowledge funding by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under SPP 1798.
A.S.\ acknowledges funding by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) under Germany's Excellence Strategy – MATH+ : The Berlin Mathematics Research Center, EXC-2046/1 – project ID: 390685689.

==> sec_MultiBit.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Proof
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/TranslationInvariance.pdf}
    \caption{Two points remain separated by the multi-bit measurement $\a_i$ when translated as long as the translation remains within the range of the quantizer. \red{(put to TikZ)}}
    \label{fig:translation}
\end{figure}

\section{Proof of Multi-Bit \red{(To Be Moved into Proof Section)}}
The proof will is related to the 1-bit case. The main difference is that
in the multi-bit case we present proofs for two differenc regimes, which
are defined by the resolution $\Delta$ of the quantizer $Q: \R^m \to 
\mathcal{A}_{\Delta,B}^m$ and the desired accuracy $\rho>0$. Indeed, if the 
desired accuracy satisfies $\rho \geq c_0 \Delta$, then we show that the
number of measurements $m$, which are necessary in order to recover a 
low complexity signal $x \in \R^n$ from its quantized measurements scale
like in classical compressive sensing scenario, i.e., it behaves like
there is no quantization. In the contrary, if one tries to achive an accuracy
$\rho>0$, such that $\rho < \Delta$, then we essentially observe the
same behavior as in the $1$-bit case, which was discussed in section~TODO.

The argument presented to make the two regimes visible essentially follows
the argument presented in the $1$-bit case. Working above the quantizer
resolution requires a change of gears when one tries to extend
the point-wise results to uniform results in $\T \subset \R^n$. We essentially
only extend the point-wise estimates to a small localized subset of $\T$ 
and then use the elementary property of multi-bit quantization, that it behaves 
locally on small scales everywhere in the same way, i.e., translation invariant, see 
Figure~\ref{fig:translation}.

\subsection{Multi-bit Compressive Sensing above the quantizer resolution}

We start with generalizing the concept of well-separating hyperplanes from the 
one-bit to the multi-bit setting.

\begin{definition}
    We say that $H_{\a_i}$ well-separates $\x,\y \in \R^n$ if there exists $j' \in \{-(2^{B-1}-1),...,(2^{B-1}-1)\}$ such that:
    \begin{itemize}
        \item $Q_{i,j'}(\x) \neq Q_{i,j'}(\y)$
        \item $|\langle \a_i,\x \rangle + (\tau_i + j'\Delta)| \ge \theta \norm{\x - \y}{2}$
        \item $|\langle \a_i,\y \rangle + (\tau_i + j'\Delta)| \ge \theta \norm{\x - \y}{2}$
    \end{itemize}
\end{definition}

The following lemma which generalizes Theorem \ref{thm:well-separating} to multi-bit 
measurements is the core of the argument. It states that as long as two points 
have a distance of at least $3\Delta$ there is no influence of the resolution onto 
the number of measurements sufficient to have well-separation.

\begin{lemma} \label{lem:multi_bit_separation}
Let $R,\Delta>0$ and let $\x,\y \in R B_2^n \subset \R^n$ such that 
$\norm{\x-\y}{2} \geq 3 \Delta$. Further, let $\mathcal{A}_{\Delta,B}^m$ denote 
a quantization alphabet as defined in \eqref{eq:Alphabet} such that $(2^B-1)\Delta 
\ge cR$, for some constant $c \ge 1$ only depending on the subgaussian norm $L$ of 
the rows of $\A$, and let $q: \R^m \to \mathcal{A}_{\Delta,B}^m$ denote the 
corresponding quantizer. Then there are absolute constants $c_1,c_2 > 0$, which only 
depend on $\theta \in (0,1)$ and $L$, such that with probability at least $1-5e^{-c_1 m}$
    \begin{align*}
        |I(\x,\y,\theta)| \ge c_2 m,
    \end{align*}
where $I(\x,\y,\theta)$ denotes the set of indices $i$ such that $\a_i$ well-separates 
$\x$ and $\y$.
\end{lemma}

To proof this lemma we rely on the relation $ q(\x) = Q(\x) \mathbbm{1} \frac{\Delta}{2}$. 
Indeed, for $\a, \x,\y\in \R^m$ the function $|q(\inner{\a}{\x}) - q(\inner{\a}{\y})|$ 
essentially (up to a factor $2/\Delta$) counts the number of hyperplanes with normal 
direction $\a$ separating the points $\x$ and $\y$. This observation is vital to 
the following argument.

\begin{lemma} \label{lem:multi_bit_sep}
    Let $N(\x,\y,\a_i)$ denote the number of hyperplanes separating $\x$ and $\y$ 
    in direction $\a_i$ and define
    \begin{equation}
	    \label{eq:definition_J_set}
        J(\x,\y,\beta) := \{i \in [m] : 
        N(\x,\y,\a_i) \geq \beta \Delta^{-1} \norm{\x-\y}{2} \}
    \end{equation}
    Under the assumptions of Lemma \ref{lem:multi_bit_separation}, there are absolute 
    constants $c_1,c_2 > 0$, which only depend on $\beta>0$ and $L$, such that
    with probability at least $1-5\exp(-c_1 m)$
    \begin{equation}
        |J(\x,\y,\beta)| \geq c_2 m.
    \end{equation}
\end{lemma}

Before we give a proof of Lemma \ref{lem:multi_bit_separation} we observe the 
following fact, which follows by a standard calculation.

\begin{lemma} \label{lem:expectation_quantizer}
Let $C>0$ and $\langle \a_i,\x \rangle, \langle \a_i,\y \rangle \in [-C,C] \subset 
\R$. For $\Delta >0$ let $\mathcal{A}_{\Delta,B}$ denote a quantization alphabet 
as defined in \eqref{eq:Alphabet} such that $C \leq (2^B-1)\Delta$ and let $q: \R 
\to \mathcal{A}_{\Delta,B}$ denote the corresponding one dimensional quantizer. If 
$\tau_i \sim \unif([-\Delta,\Delta])$, then for all $i \in [m]$
    \begin{align*}
        \E_{\tau_i} [q(\x)_i] = \langle \a_i,\x \rangle \; ,
    \end{align*}
and in particular
    \begin{align*}
        \E_{\tau_i} [| q(\x)_i - q(\y)_i |] = |\langle \a_i, \x - \y \rangle| \; .
    \end{align*}
\end{lemma}

\begin{proof}
    \red{Give proof and put to Appendix!}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:multi_bit_sep}]
We introduce the normalized random variables $Z_i:=\frac{2}{\Delta}|q(\x)_i-
q(\y)_i|$, which count the number of hyperplanes separating $\x$ and $\y$ and we 
observe that by Lemma \ref{lem:expectation_quantizer} we have $\E_{\tau_i} [Z_i] 
= \frac{2}{\Delta} |\inner{\a_i}{\x} - \inner{\a_i}{\y}|$ provided that 
$|\inner{\a_i}{\x}|,|\inner{\a_i}{\y}|\leq cR$. We are interested in the events
\begin{equation}
    E_i = \{Z_i \geq \beta \norm{\x-\y}{2} \Delta^{-1} \} \; .
\end{equation}
If we can show that $\sum_{i=1}^m \1_{E_i} \geq c_2 \Delta^{-1} \norm{\x-\y}{2} m$, 
the result follows. To do so, we first restrict ourselves to measurements $\a_i$ 
which behave well in the sense that the projections of $\x$ and $\y$ onto $\a_i$ 
are bounded by $cR$ and that the hyperplane $H_{\a_i}$ is quite orthogonal to the 
connecting line between $\x$ and $\y$. Let us denote this set by
\begin{equation*}
I:=\Big\{i\in [m]\; : \; \max\{|\inner{\a_i}{\x}|,|\inner{\a_i}{\y}|\} \leq 
\frac{4R}{\sqrt{\ep}}\text{ and } |\inner{\a_i}{\x-\y}| \geq 
\gamma \norm{\x-\y}{2} \Big\},
\end{equation*} 
where $\eps \in (0,1)$ will be determined below. By the Paley-Zygmund inequality, 
for any $\gamma\in (0,1)$ we have
\begin{displaymath}
 \mathbb{P}(|\inner{\a_i}{\x-\y}|^2 \geq \gamma^2 
\norm{\inner{\a_i}{\x-\y}}{L_2}^2) \geq (1-\gamma^2)^2 
\frac{\norm{\inner{\a_i}{\x-\y}}{L^2}^4}{\norm{\inner{\a_i}{\x-\y}}{L^4}^4}.
\end{displaymath}
Since $\a_i, i=1,...,m$ are subgaussian we have $\norm{\inner{\a_i}{\x-\y}}{L^4} 
\leq 2 L\norm{\inner{\a_i}{\x-\y}}{L^2}$ and therefore by isotropy
\begin{displaymath}
 \mathbb{P}(|\inner{\a_i}{\x-\y}| \geq \gamma 
\norm{\x-\y}{2}) \geq (1-\gamma^2)^2 \frac{1}{(2L)^4} \; .
\end{displaymath}
Setting $\ep:=(1-\gamma^2)^2 \frac{1}{(2L)^4}\in (0,1)$ we obtain
\begin{equation} \label{eq/small_ball_condition}
  \mathbb{P}(|\inner{\a_i}{\x-\y}| \geq \gamma 
\norm{\inner{\a_i}{\x-\y}}{L_2}) \geq \ep .
\end{equation}
Further, note that the subgaussian random variables $\inner{\a_i}{\x}$ 
are square integrable. Hence, by isotropy and Chebychev's inequality, the 
following holds for $\ep' \in (0,1)$
\begin{displaymath}
 \mathbb{P}(|\inner{\a_i}{\x}| \geq \norm{\x}{2} /\sqrt{\ep'}) \leq \ep' \; .
\end{displaymath}
Considering the $m$ independent rows $\a_i$ of $\A$ a Chernoff bound reveals that
\begin{displaymath}
 | \{ i \in [m] \; : \; |\inner{\a_i}{\x}| \geq \norm{\x}{2}/\sqrt{\ep'} 
\}| 
\leq 2 \ep' m
\end{displaymath}
holds with probability at least $1 - 2 \exp(-c_1 \ep' m)$. 
Applying the small ball condition in \eqref{eq/small_ball_condition} to 
a sequence $(\a_i)_{i \in [m]}$ another Chernoff bound yields, that with probability 
at least $1- 2 \exp(-c_1\ep m)$ we have
\begin{equation}
 |\{i \in [m] \; : \; |\inner{\a_i}{\x-\y}| \geq \gamma 
\norm{\x-\y}{2}\}| \geq \frac{\ep m}{2} \; .
\end{equation}
Choosing $\ep' := \ep/16$ we get that with $\A$-probability at least $1- 4\exp(-c_1
\ep m)$ the set $I$ satisfies $|I|\geq \frac{\ep m}{4}$. Let us restrict ourselves 
to measurements indexed in $I$ for the rest of the proof.\\
By applying Payley-Zygmund to the random variable $Z_i$, we get for any $\theta 
\in (0,1)$ that  
 \begin{equation} \label{eq:Ptau}
  \mathbb{P}_{\tau_i}\Big(Z_i \geq \theta \E [Z_i] \Big) \geq (1-\theta)^2 
  \frac{\E [Z_i]^2}{\E [Z_i^2]} \; .
 \end{equation}
By $|\inner{\a_i}{\x}-\inner{\a_i}{\y}| \geq \gamma \norm{\x-\y}{2}> 2 \Delta$, 
for $\gamma > \frac{2}{3}$, we have that
\begin{align*}
 Z_i &\leq \frac{|(\inner{\a_i}{\x} + \tau_i)-(\inner{\a_i}{\y} 
 	+ \tau_i)|}{2\Delta} +1 \\
 &\leq \frac{|(\inner{\a_i}{\x} + \tau_i)-(\inner{\a_i}{\y} + \tau_i)|}{2\Delta} 
 + \frac{|(\inner{\a_i}{\x} + \tau_i)-(\inner{\a_i}{\y} + \tau_i)|}{2\Delta} \\
 &= \frac{|\inner{\a_i}{\x}-\inner{\a_i}{\y}|}{\Delta}  \; .
\end{align*}
Hence, the choice $\theta = \frac{1}{2}$ in \eqref{eq:Ptau} together with 
$|\inner{\a_i}{\x}-\inner{\a_i}{\y}|\geq \gamma \norm{\x-\y}{2}$ leads to
\begin{equation*}
  \mathbb{P}_{\tau_i} \Big(Z_i \geq \gamma \Delta^{-1} \norm{\x - \y}{2} \Big) 
  \geq \frac{1}{4} \frac{\E [Z_i]^2}{\E [Z_i^2]} 
  \geq \frac{1}{4} \frac{\Delta}{|\inner{\a_i}{\x}-\inner{\a_i}{\y}|} 
  	\frac{\E [Z_i]^2}{\E [Z_i]} = \frac{1}{8}.
\end{equation*}
An additional Chernoff bound yields now that with $\ttau$-probability at least 
$1-\exp(-c_1m)$
\begin{equation}
    \sum_{i=1}^m \1_{\{Z_i \geq \norm{\x-\y}{2} \Delta^{-1} \beta\} } \geq c_2 m \; .
\end{equation}
A union bound over the $\A$- and the $\ttau$-event concludes the proof.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:multi_bit_separation}]
The statement follows directly from Lemma \ref{lem:multi_bit_sep}. Just note that 
if, for some $i \in [m]$, we have $N(\x,\y,\a_i) \geq \beta \norm{\x-\y}{2} 
\Delta^{-1}$, then there is $j \in \{-(2^{B-1}-1),...,(2^{B-1}-1)\}$, such that
    \begin{equation}
        |\inner{\a_i}{\x} + \tau_i + j \Delta| \geq \kappa \norm{\x-\y}{2}
        \text{ and }
        |\inner{\a_i}{\y} + \tau_i + j \Delta| \geq \kappa \norm{\x-\y}{2} \; ,
\end{equation}
where one uses the assumption that the quantizers range covers the whole 
interval $[-R,R]$.
\end{proof}

\paragraph{Localized uniform result} Define $T_\Delta = (T-T)\cap 12\Delta B_2^n$. 
By arguing similarly to the one-bit case, we can obtain the following uniform result.

\begin{theorem} \label{thm:LocalMultiBit}
    Assume that
    \begin{align*}
        m \gtrsim w(T_\Delta) + \log(|N_\Delta|).
    \end{align*}
    Then with probability at least $1-2e^{-cm}$ we have for all $\x,\y \in T_\Delta$ 
    with $\norm{\x - \y}{2} \ge 12 \Delta$ that
    \begin{align*}
        |I(\x,\y,\theta)| \ge \frac{c'}{2} m.
    \end{align*}
\end{theorem}

\begin{proof}
First note that if $\frac{c_1}{\sqrt{m}} (w(T_\Delta) + \Delta \sqrt{m}) \le \rho$,
for $\rho > 0$, then with probability at least $1 - e^{-c_0m}$ one has by 
Lemma~\ref{lem:bound_for_spoiled_hyperplanes} that
    \begin{align*}
        \sup_{\z \in T_\Delta} |\{ i \in [m] \colon |\langle \a_i,\z \rangle| 
	\ge \rho \}| \le \frac{c'}{4} m.
    \end{align*}
Moreover, if $N_\Delta$ is a $2\Delta$-net of $T_\Delta$, we get by a simple union 
bound that with probability at least $1 - |N_\Delta|^2 e^{-cm}$, for all $\x',\y' 
\in N_\Delta$,
    \begin{align*}
        |I(\x',\y',\theta)| \ge c'm \Delta^{-1} \norm{\x' - \y'}{2} \ge c'm.
    \end{align*}
We can now apply Lemma \ref{lem:noise_stability} with $\rho = 8\Delta$ and $\eps = 2\Delta$ 
to get for all $\x',\y' \in N_\Delta$ with $\norm{\x' - \y'}{2} \ge 8\Delta$ and 
all $\x,\y$ with $\norm{\x - \x'}{2} \le 2\Delta$ and $\norm{\y - \y'}{2} \le 2\Delta$ 
that
    \begin{align*}
        |I(\x,\y,\theta/2)| \ge |I(\x',\y',\theta)| - \frac{c'}{4} m \ge \frac{c'}{2} m
    \end{align*}
which yields the claim by a union bound over the two above events.
\end{proof}

\paragraph{Extension to the whole set} We will use now the elementary properties 
of our uniform multi-bit quantizer to extend Theorem \ref{thm:LocalMultiBit} to 
the complete signal set $T$.

\begin{theorem} \label{thm:MultiBit}
    Assume that
    \begin{align*}
        m \gtrsim w(T_\Delta) + \log(|N_\Delta|).
    \end{align*}
    Then with probability at least $1 - 2e^{-cm}$ we have for all $\x,\y \in T$ 
    with $\norm{\x - \y}{2} \ge 12 \Delta$ that
    \begin{align*}
        \left| I\left(\x,\y,\frac{\Delta}{2 \norm{\x - \y}{2}} \right) \right| 
	\ge \frac{c'}{4} m.
    \end{align*}
\end{theorem}

\begin{proof}[Proof of Theorem \ref{thm:MultiBit}]
    By Theorem \ref{thm:LocalMultiBit} we get for all $\x,\y \in \T$, such that 
    $\norm{\x - \y}{2} = 12\Delta$ with probability at least $1-2e^{-cm}$ that
    \begin{align*}
        |I(\0,\x-\y,\theta/2)| \ge \frac{c'}{2}m.
    \end{align*}
    If $\norm{\x - \y}{2} > 12 \Delta$, one can by convexity of $T$ just reduce 
    the following argument to shorter segment of the connecting line. We get by 
    definition of well-separation that for all $i \in I(\0,\x-\y,\theta/2)$ there 
    exist $j_i \in \{-(2^{B-1}-1),...,(2^{B-1}-1)\}$ such that
    \begin{itemize}
        \item $Q_{i,j_i}(\0) \neq Q_{i,j_i}(\x-\y)$,
        \item $|\langle \a_i,\x - \y \rangle + (\tau_i + j_i \Delta)| 
		\ge \frac{\theta}{2} 12 \Delta$,
        \item $|\tau_i + j_i \Delta| \ge \frac{\theta}{2} 12 \Delta$.
    \end{itemize}
    This implies for $\theta \ge \frac{1}{6}$ and all $i \in I(\0,\x-\y,\theta/2)$ that
    \begin{align} \label{eq:distance}
        |\langle \a_i,\x \rangle - \langle \a_i,\y \rangle| 
	= |\langle \a_i,\x - \y \rangle + (\tau_i + j_i\Delta) 
		- (\tau_i + j_i\Delta)| \ge 12\theta \Delta 
	\ge 2\Delta.
    \end{align}
    By Lemma \ref{lem:bound_for_spoiled_hyperplanes}, we have with probability at least $1 - e^{-cm}$ that
    \begin{align*}
        |I(\0,\x-\y,\theta/2) \cap \{ i \in [m] 
	\colon \sup_{\z \in T} |\langle \a_i,\z \rangle| \le R \}| 
	\ge \frac{c'}{4}m.
    \end{align*}
    As \eqref{eq:distance} together with the assumption $(2^{B-1}-1)\Delta \ge R$ 
    guarantees for all $i \in I(\0,\x-\y,\theta/2) \cap \{ i \in [m] \colon 
    \sup_{\z \in T} |\langle \a_i,\z \rangle| \le R \}$ that there exists a $j_i'$ 
    such that
    \begin{itemize}
        \item $Q_{i,j_i'}(\x) \neq Q_{i,j_i'}(\y)$,
        \item $|\langle \a_i,\x \rangle + (\tau_i + j_i' \Delta)| \ge \frac{\Delta}{2}$,
        \item $|\langle \a_i,\y \rangle + (\tau_i + j_i' \Delta)| \ge \frac{\Delta}{2}$,
    \end{itemize}
    we obtain the claim by a union bound over the above events.
\end{proof}

\subsection{Compressive sensing beyond the quantizer resolution}
In the first part of this section we showed that the a low complexity signal $x \in \R^n$
is recovered from its quantized measurements by the program \eqref{eq:P} as long as
the desired accuracy $\rho>0$ is above the resolution of the quantizer $Q : \R^m
\to \mathcal{A}_{\Delta}$. This section deals with accuracies $\rho< c \Delta$.
The first step is to derive a point-wise estimate. Since the $\rho \leq c \Delta$,
we have the following result.

\begin{lemma} \label{lem:multi_bit_separation}
	Let $R,\Delta, \rho>0$ and let $\x,\y \in R B_2^n \subset \R^n$ such that 
	$\norm{\x-\y}{2} \geq \rho$. Further, let $\mathcal{A}_{\Delta,B}^m$ denote 
	a quantization alphabet as defined in \eqref{eq:Alphabet} such that $(2^B-1)\Delta 
	\ge cR$, for some constant $c \ge 1$ only depending on the subgaussian norm $L$ of 
	the rows of $\A$, and let $q: \R^m \to \mathcal{A}_{\Delta,B}^m$ denote the 
	corresponding quantizer. Then there are absolute constants $c_1,c_2 > 0$, which only 
	depend on $\theta \in (0,1)$ and $L$, such that with probability 
	at least $1-5 \exp(-c_1 m \norm{\x-\y}{2}/\Delta )$
    \begin{align*}
	    |I(\x,\y,\theta)| \ge c_2 m \frac{\norm{\x-\y}{2}}{\Delta},
    \end{align*}
	where $I(\x,\y,\theta)$ denotes the set of indices $i$ such that $\a_i$ well-separates 
	$\x$ and $\y$.
\end{lemma}
\begin{proof}
	Let $\beta >0$ to be specified later and let $J(\x,\y,\beta) = \{i \in [m]:
	N(\x,\y,\a_i) \geq \beta \Delta^{-1} \norm{\x-\y}{2} \}$ denote the
	set defined in \eqref{eq:definition_J_set}, where $N(\x,\y,\a_i)$ denotes
	the number of hyperplanes seperating $\x$ and $\y$ in direction $\a_i$.
	We observe that since $\norm{\x-\y}{2} \leq \Delta$ for any realization of
	$\a_i$ we have $N(\x,\y,\a_i) \in \{0,1\}$. The value of $N(\x,\y,\a_i)$ is
	determined by the event $\q( \inner{\a_i}{\x} + \tau_i) \neq \q(\inner{\a_i}{\x}
	+ \tau_i)$, i.e.,  
	\begin{equation*}
		N(\x,\y,\a_i) = 
		\begin{cases}
			1 &\text{if } 
				\q( \inner{\a_i}{\x} + \tau_i) 
				\neq \q(\inner{\a_i}{\x} + \tau_i)\; , \\
			0 &\text{if }
				\q( \inner{\a_i}{\x} + \tau_i) 
				= \q(\inner{\a_i}{\x} + \tau_i) \; .
		\end{cases}
	\end{equation*}
	Observing that 
	$$\1_{\q( \inner{\a_i}{\x} + \tau_i) \neq \q(\inner{\a_i}{\x}
	+ \tau_i)} = \frac{1}{2\Delta}  |\q( \inner{\a_i}{\x} + \tau_i) 
	- \q(\inner{\a_i}{\x} + \tau_i)|\; , $$
	it follows from Lemma~\ref{lem:expectation_quantizer} that 
	\begin{equation}
		\P_{\tau}(\q( \inner{\a_i}{\x} + \tau_i) 
		\neq \q(\inner{\a_i}{\x} + \tau_i) )
		= \frac{1}{2\Delta} | \inner{\a_i}{\x-\y}| \; .
	\end{equation}
	Recall from the proof of Lemma~\ref{lem:multi_bit_sep} that for any $\ep>0$
	and a suitiable constant $\gamma >0$ the set	
	\begin{equation*}
	I:=\Big\{i\in [m]\; : \; \max\{|\inner{\a_i}{\x}|,|\inner{\a_i}{\y}|\} 
	\leq \frac{4R}{\sqrt{\ep}}\text{ and } |\inner{\a_i}{\x-\y}| \geq 
	\gamma \norm{\x-\y}{2} \Big\},
	\end{equation*} 
	satisfies $|I|\geq \frac{\ep m}{4}$ with $\A$-probability $1-\exp(-c_1 \ep m)$.
	On this event we have
	\begin{equation}
		\P(\q( \inner{\a_i}{\x} + \tau_i) 
		\neq \q(\inner{\a_i}{\x} + \tau_i) )
		\geq \frac{\gamma}{2\Delta} \norm{\x-\y}{2} \; . 
	\end{equation}
	Hence, a Chernoff bound shows that 
	with $(\tau_i)_{i \in [m]}$-probability 
	$1-\exp(- c' m \norm{\x-\y}{2}/\Delta)$ we have
	\begin{equation}
		\label{eq:chernoff_bound_for_multi_bit}
		\sum_{i=1}^m \1_{\q( \inner{\a_i}{\x} + \tau_i) 
			\neq \q(\inner{\a_i}{\x} + \tau_i)} 
		\geq \frac{c m \norm{\x-\y}{2}}{\Delta}
	\end{equation}
	Combing the event $|I| \geq \frac{\ep m}{4}$ with the event in
	\eqref{eq:chernoff_bound_for_multi_bit} it follows that for suitiable
	$\beta(\theta)>0$, we have
	\begin{equation}
		|I(\x,\y,\theta)| \geq \frac{c_0 m \norm{\x-\y}{2}}{\Delta} \; .
	\end{equation}
	This conculdes the proof. 
\end{proof}
We are left with lifting this estimate to the set $\T$. The argument is similar to
the one bit case. We can directly use a modified version of Lemma~\ref{lem:stability}. 

\begin{lemma}[Stability of separating hyperplanes]
\label{lem:multi_bit_stability}
Let $\x',\z' \in \T \subset \R^n$ such that $\norm{\x'-\z'}{2} \geq
\rho$. Assume that $\ep \leq \rho/4 \leq \Delta$ and suppose that
\begin{equation}
\label{eqn:mb_small_spoiling_set}
    \sup_{\y\in (\T-\T)\cap \ep B^n_2}|\{i\in [m]\; : \; 
    |\inner{\a_i}{\y}|>\kappa \rho/4\}|\leq k \; ,
\end{equation}
where $\kappa>0$ is some constant.
Then, for all $\x, \z \in \T$ satisfying $\norm{\x-\x'}{2} \leq \ep$ and $\norm{\z-\z'}{2} \leq \ep$, we have
\begin{equation}
    |I(\x,\z,\kappa/2)| \geq |I(\x',\z',\kappa)|  - 2k \;.
\end{equation}
\end{lemma}
The proof directly follows from the proof of Lemma~\ref{lem:stability}. This result leads to a multi-bit version of Theorem~\ref{thm:uniform}. 
%TODO state the result
\red{State the result, finish the argument}
